Multilevel Monte Carlo with Numerical Smoothing for Robust and Efficient Computation of Probabilities and Densities

The multilevel Monte Carlo (MLMC) method is highly efficient for estimating expectations of a functional of a solution to a stochastic differential equation (SDE). However, MLMC estimators may be unstable and have a poor (noncanonical) complexity in the case of low regularity of the functional. To overcome this issue, we extend our previously introduced idea of numerical smoothing in (Quantitative Finance, 23(2), 209-227, 2023), in the context of deterministic quadrature methods to the MLMC setting. The numerical smoothing technique is based on root-finding methods combined with one-dimensional numerical integration with respect to a single well-chosen variable. This study is motivated by the computation of probabilities of events, pricing options with a discontinuous payoff, and density estimation problems for dynamics where the discretization of the underlying stochastic processes is necessary. The analysis and numerical experiments reveal that the numerical smoothing significantly improves the strong convergence, and consequently, the complexity and robustness (by making the kurtosis at deep levels bounded) of the MLMC method. In particular, we show that numerical smoothing enables recovering the MLMC complexities obtained for Lipschitz functionals due to the optimal variance decay rate when using the Euler--Maruyama scheme. For the Milstein scheme, numerical smoothing recovers the canonical MLMC complexity even for the nonsmooth integrand mentioned above. Finally, our approach efficiently estimates univariate and multivariate density functions.

==> Conclusion.tex <==
In this work,  we propose  novel approaching for smoothing  , fast option pricers,  for options whose underlyings  follow the rBergomi model, as in \cite{bayer2016pricing}.  The new methods  are based on hierarchical deterministic quadrature methods:  i) ASGQ using the same construction as in \cite{haji2016multi}, and ii) the QMC method. Both techniques are coupled with a Brownian bridge construction and the Richardson extrapolation on the weak error.

Given that the only prevalent option, in this context, is to use different variants of the MC method, which is computationally expensive, our main contribution  is to propose a competitive alternative to the MC approach that is based on deterministic quadrature methods.  We believe that we are the first to propose (and design) a pricing method, in the context of rough volatility models, that is based on deterministic quadrature, and that  our approach  opens a new research direction  to investigate the performance of other methods besides MC, for pricing and calibrating under rough volatility models. 

Assuming one targets price estimates with a sufficiently small relative error tolerance, our proposed methods demonstrate substantial computational gains  over the standard MC method, when pricing under the rBergomi model, even for very small values of the Hurst parameter. We show  these gains through our numerical experiments for  different parameter constellations.  We clarify that we do not claim that these gains will hold in the asymptotic regime, i.e.,  for higher accuracy requirements. Furthermore, the use of the Richardson extrapolation is justified in the pre-asymptotic regime, for which our observed experimental results suggest a convergence of order one for the weak error. We emphasize that, to the best of our knowledge, no proper weak error analysis has been done in the rough volatility context, but we claim that both hybrid and exact schemes have  a weak error  of order one, which is justified, at least numerically.  While our focus is on the rBergomi model, our approach is applicable to a wide class of stochastic volatility models, in particular rough volatility models.

In this work, we limit ourselves to compare our novel proposed method against the standard MC. A more systematic comparison against the variant of MC proposed in \cite{mccrickerd2018turbocharging}  can be carried out, but this remains for a future study. Another future research direction is to provide a reliable method for controlling the quadrature error for ASGQ which is,  to the best of our knowledge,  still  an open research problem. This is even more challenging in our context, especially for low values of $H$. We emphasize that the main aim of this work is to illustrate the high potential of the deterministic quadrature, when coupled with hierarchical representations, for pricing options under the rBergomi model. Lastly, we note that accelerating  our novel  approach can be achieved  by using better versions of the ASGQ and QMC methods or an alternative weak approximation of rough volatility models, based on a Donsker type approximation, as recently suggested in \cite{horvath2017functional}. The ASGQ and QMC methods proposed in this work can also be applied in the context of this scheme; in this  case, we only have an $N$-dimensional input rather than a ($2N$)-dimensional input for the integration problem  \eqref{BS_formula_rbergomi_2}, with $N$ being the number of time steps. Further analysis, in particular regarding the Richardson approximation, will be done in future research.


==> More_details_numerical_smoothing.tex <==
\subsection{Extension to the high dimensional case}
In the high dimensional case, we denote by $(z_1^{(i)},\dots,z_N^{(i)})$ the $N$ Gaussian independent rdvs that will be used to construct the path of the $i$-th asset $\bar{X}^{(i)}$, where $1 \le i \le d$ ($d$ denotes the number of underlyings considered in the basket). We keep the  same notations by denoting  $\psi: (z_1^{(i)},\dots,z_N^{(i)}) \rightarrow (B_1,\dots,B_N)$ the mapping of Bb construction and by $\Phi: (B^{(i)}_1,\dots,B^{(i)}_N) \rightarrow \bar{X}^{(i)}_T$, the mapping consisting of the time-stepping scheme. Then, we can express the option price as
\begin{align*}
	\expt{g(\mathbf{X}(T))}&\approx	\expt{g\left(\Phi \circ \psi \right) (z_1^{(1)}, \dots, z_N^{(1)}, \dots, z_1^{(d)},\dots,z^{(d)}_N)} \nonumber\\
	&=\int_{\rset^{d \times N}} G(z_1^{(1)}, \dots, z_N^{(1)}, \dots, z_1^{(d)},\dots,z^{(d)}_N)) \rho_{d \times N}(\mathbf{z}) dz_1^{(1)} \dots dz_N^{(1)} \dots z_1^{(d)} \dots dz^{(d)}_N \COMMA
\end{align*}
where $G=g \circ \Phi \circ \psi$ and
\begin{equation*}
\rho_{d \times N}(\mathbf{z})=\frac{1}{(2 \pi)^{{d \times N}/2}} e^{-\frac{1}{2} \mathbf{z}^T \mathbf{z}} \PERIOD
\end{equation*}
Now,  performing the  pre-integrating step with respect to the coarse rdvs $(z_1^{(1)},\dots, z_1^{(d)} )$, results in
\begin{small}
\begin{align}\label{eq: pre_integration_step_wrt_y1_basket}
	\expt{g(\mathbf{X}(T))}&=\int_{\rset^{d \times N}} G(z_1^{(1)}, \dots, z_N^{(1)}, \dots, z_1^{(d)},\dots,z^{(d)}_N)) \rho_{d \times N}(\mathbf{z}) dz_1^{(1)} \dots dz_N^{(1)} \dots z_1^{(d)} \dots dz^{(d)}_N \nonumber\\ 
	&=\int_{\rset^{d \times (N-1)}} \left(\int_{\rset^d} G(z^{(1)}_1,\mathbf{z}^{(1)}_{-1},\dots,z^{(d)}_1,\mathbf{z}^{(d)}_{-1} ) \rho_d(z_1^{(1)},\dots,z_1^{(d)}) dz_1^{(1)}\dots dz_1^{(d)}  \right) \rho_{d \times(N-1)}(\mathbf{z}_{-1}^{(1)},\dots,\mathbf{z}_{-1}^{(d)}) d\mathbf{z}_{-1}^{(1)}\dots d\mathbf{z}_{-1}^{(d)}\nonumber\\	
	&=\int_{\rset^{d\times (N-1)}} h(\mathbf{z}^{(1)}_{-1},\dots,\mathbf{z}^{(d)}_{-1} ) \rho_{d\times (N-1)}(\mathbf{z}_{-1}^{(1)},\dots,\mathbf{z}_{-1}^{(d)}) d\mathbf{z}^{(1)}_{-1} \dots d\mathbf{z}^{(d)}_{-1}\COMMA \\ \nonumber
	&=\expt{h(\mathbf{z}^{(1)}_{-1},\dots,\mathbf{z}^{(d)}_{-1} )}
\end{align}
\end{small}
where $h(\mathbf{z}^{(1)}_{-1},\dots,\mathbf{z}^{(d)}_{-1})=\int_{\rset^d} G(z^{(1)}_1,\mathbf{z}^{(1)}_{-1},\dots,z^{(d)}_1,\mathbf{z}^{(d)}_{-1} )   \rho_d(z_1^{(1)},\dots,z_1^{(d)}) dz_1^{(1)}\dots dz_1^{(d)}$.


==> Numerical_experiments.tex <==
In this section, we conduct our experiments for three different examples of payoffs: i)  a single digital option, ii) a single call option, and iii) a $4d$-basket call option. The three examples are tested under two different dynamics for the asset price: i)  the discretized GBM model (a didactic example), and ii) the  discretized Heston model, which is a relevant application of our approach. 
\begin{remark}
Although, the discretization of the GBM dynamics is not needed for some of the examples that we consider.  We emphasize that we aim to show the efficiency of our proposed approach for dynamics where discretization is required, such as the Heston model that we test in this work. On the other hand, examples under the GBM are only considered here as instructive examples to showcase our approach.
\end{remark}
For each example, we estimate the weak error (Bias) of MC, then we conduct a comparison between MC and ASGQ in terms of errors and computational time.  While fixing  a  sufficiently small error tolerance in the price estimates,  we  compare the computational time needed for both methods to meet the desired error tolerance.  For all our numerical experiments, the  reported errors are relative errors, normalized by the reference solutions. Furthermore, we conduct our numerical experiments for two different scenarios: i) without Richardson extrapolation, and ii) with level $1$ of the Richardson extrapolation. We note that  in all cases the actual work (runtime) is obtained using an Intel(R) Xeon(R) CPU E$5$-$268$ architecture. 

We show  the summary of our numerical findings in Table \ref{table:Summary of our numerical results.}, which  highlights the computational gains achieved by ASGQ combined with numerical smoothing compared to the  MC method to meet a certain error tolerance, which we set approximately below  $1\%$. We note that the results are reported using the best configuration with Richardson extrapolation for each method. More detailed results for each case  are provided in  Sections \ref{sec:Results for the binary option example}, \ref{sec:Results for the call option example}, \ref{sec:The basket call option  under GBM  model}, \ref{sec:Digital option under the discretized  Heston model with parameters of Set 1}, and \ref{sec:European call option  under the discretized  Heston model with parameters of Set 1}.
	\begin{small}
\begin{table}[!h]
	\centering
	\begin{tabular}{l*{4}{c}r}
	\toprule[1.5pt]
		Example            &  Total relative error  & CPU time  $\left( \text{ASGQ} / \text{MC}\right)$ in \% \\
		\hline
			  Single  digital option (GBM)  &  $0.7 \%$&  $ 0.7\%$ \\	
              \hline
            Single call option (GBM)      &  $0.5\%$&  $0.8\%$ \\
%            & level $1$ &  $$ &  $$ \\		
%				 \hline
%					$2d$-Basket call option (GBM)  & without    &  $$0.9\%$$&  $4.8\%$ \\	
					\hline
					$4d$-Basket call option (GBM)     &  $0.8\%$&  $7.4\%$ \\	
					\hline
					  Single  digital option (Heston)   &$0.6\%$&  $6.2\%$ \\	
              \hline
					  Single call option (Heston)   &  $0.5\%$&  $17.2\%$ \\
%					  \hline
%					  $4d$-Basket call option (Heston)   &  $.$&  $.$ \\	
		\bottomrule[1.25pt]
	\end{tabular}
	\caption{Summary of relative errors and computational gains, achieved by ASGQ combined with numerical smoothing, compared to the MC method,  to meet a certain error tolerance.  We note that the ratios are computed for the best configuration with Richardson extrapolation for each method.}
	\label{table:Summary of our numerical results.}
\end{table}
\end{small}
%Along the numerical part below, we compare $3$ methods:
%\begin{enumerate}
%\item[i)] ASGQ based on construction as explained in Section \ref{sec:Details of the ASGQ}.
%\item[ii)] Plain Monte Carlo where we apply standard Monte Carlo and we refer to it by "MC".
%\item[iii)] Monte Carlo applied to the smoothed payoff function after numerical smoothing and we refer to it by "MC+ Num smoothing".
%\end{enumerate}

%Through our  numerical experiments, we follow these steps to achieve our reported results
%\begin{enumerate}
%\item[i)] For a fixed number of time steps, $N$, we compute an accurate estimate, using a large number of samples, $M$, of the biased  MC solution. This step also provides us with an estimate of the bias error, $\mathcal{E}_B(N)$, defined by \eqref{eq:total_error}. 
%\item[ii)] The estimated  biased solution is used as a reference solution  to ASGQ to compute the quadrature error, $\mathcal{E}_Q(\text{TOL}_{\text{ASGQ}},N)$.
%\item[iii)] In order to compare with MC method, the number of samples, $M$, is chosen so that  the statistical error  of the Monte Carlo  method, $\mathcal{E}_S(M)$, satisfies, given  total error $\mathcal{E}_{\text{tot}}$ 
%\begin{small}
%\begin{align}\label{optimal_number_samples}
%\mathcal{E}_S(M)= \mathcal{E}_B(N)=\frac{\mathcal{E}_{\text{tot}}}{2}\COMMA
%\end{align}\end{small}
%\end{enumerate}

\subsection{Options under the discretized GBM model}\label{sec:The discretized 1D Black-Scholes}
In this section,  we are interested in the  one dimensional lognormal example where, given a standard one-dimensional Brownian motion $\{W_t, 0 \leq t \leq T\} $,   the dynamics of the stock are represented by
\begin{align*}
%\label{lognormal_dynamics}
	dX_t=\sigma X_t dW_t.
\end{align*}
%In the discrete case, the numerical approximation of $X$, using $N$ time steps ($\Delta t=\frac{T}{N}$), satisfies
%%\begin{small}
%%\begin{align}
%%	\bar{X}_{t_1}&= \bar{X}_{t_0} \left[ 1+\frac{\sigma}{\sqrt{T}} Z_1 \Delta t+ \sigma \Delta B_0\right]\nonumber\\
%%	%=X_{t_0} \left[ 1+\sigma \Delta W_0 \right] \nonumber\\
%%	\bar{X}_{t_2}&= \bar{X}_{t_1} \left[ 1+\frac{\sigma}{\sqrt{T}} Z_1 \Delta t+ \sigma \Delta B_1\right]\nonumber\\
%%%	=X_{t_1} \left[ 1+\sigma \Delta W_1 \right] \nonumber\\
%%	\vdots &= \vdots\nonumber\\
%%%	 =\vdots \nonumber\\
%%	\bar{X}_{t_N}&= \bar{X}_{t_{N-1}} \left[ 1+\frac{\sigma}{\sqrt{T}} Z_1 \Delta t+ \sigma \Delta B_{N-1}\right]
%%	%= X_{t_{N-1}}  \left[ 1+\sigma \Delta W_{N-1} \right],
%%\end{align}
%%\end{small}
%%implying that
%\begin{align}\label{eq:discrete_path_expression}
%\bar{X}\left(T; Z_1, \{\Delta B_{n}\}_{n=0}^{N-1}\right)=X_0 \prod_{n=0}^{N-1} \left[ 1+\frac{\sigma}{\sqrt{T}} z_1 \Delta t+ \sigma \Delta B_{n}\right].
%\end{align}
%where $Z_1$ is a standard Gaussian rdv, and $\{\Delta B_{n}\}_{n=0}^{N-1}$ are the Brownian bridge increments. 
%
%As explained in Section \ref{sec:Discrete time, practical motivation}, the first step of our approach is determining the location of the non-smoothness. In the following, we want to compare different ways for identifying the location of the kink for this model.
%
%\subsubsection*{Exact location of the kink for the continuous problem}
%Let us denote $y^{\ast}$ an invertible function that satisfies 
%\begin{align}\label{eq: kink_point_problem}
%	\bar{X}\left(T;y^{\ast}(x),B_{[0,T]}\right)=x,
%\end{align}
%where $B_{[0,T]}$ is the Brownian bridge path.
%
%We can easily prove that the expression of $y^{\ast}$ for model given by \eqref{lognormal_dynamics} is given by
%\begin{align}
%	y^{\ast}(x)=\left(\operatorname{log}(x/x_0)+T \sigma^2/2\right) \frac{1}{\sqrt{T} \sigma}, 
%\end{align}
%and since the kink for most of options   occurs at $x=K$, where $K$ is the strike price then  the exact location of the continuous problem is given by 
%\begin{align}\label{xact_location_continuous_problem}
%	y^{\ast}(K)=\left(\operatorname{log}(K/x_0)+T \sigma^2/2\right) \frac{1}{\sqrt{T} \sigma}.
%\end{align}
%\subsubsection*{Location of the kink for the discrete problem}
%Giving \eqref{eq:discrete_path_expression}, in order to determine $y^{\ast}$, we need to solve numerically
%\begin{align}
%	x=\bar{X}\left(T;y^{\ast}(x),\{\Delta B_{n}\}_{n=0}^{N-1}\right)=X_0 \prod_{n=0}^{N-1} \left[ 1+\frac{\sigma}{\sqrt{T}} y^{\ast}(x) \Delta t+ \sigma \Delta B_{n}\right],
%\end{align}
%which implies that the location of the kink point for the approximate problem is equivalent to finding the roots of the polynomial $P(y^\ast(x))$, given by
%\begin{align}\label{polynomial_kink_location}
%	P(y^{\ast}(x))=\prod_{n=0}^{N-1} \left[ 1+\frac{\sigma}{\sqrt{T}} y^\ast(x) \Delta t+ \sigma \Delta B_{n}\right]-\frac{x}{X_0}.
%\end{align}
%The  location of the kink can be obtained  by solving the root finding problem: $P(y^{\ast}(x))=0$.  In this work, we try to  find the roots of polynomial $P(y^{\ast}(x))$, given by \eqref{polynomial_kink_location}, by using Newton iteration method,  with a Newton tolerance that we denote $TOL_{\text{Newton}}$. We  decompose the total integration domain   into sub-domains such that the integrand is smooth in the interior of each sub-domain  and such that the kink is located along the boundary of these areas. The total integral,  is then given as the sum of the separate integrals as expressed in \eqref{eq:smooth_function_after_pre_integration}.
%
%
%%In this case, we need the expression $P'=\frac{d P}{d y^\ast}$. If we denote $f_i(y)=1+\frac{\sigma}{\sqrt{T}} y \Delta t+ \sigma \Delta B_{i}$, then we can easily show that
%%\begin{align}\label{polynomial_kink_location_derivative}
%%	P'(y)=\frac{\sigma \Delta t}{\sqrt{T}} \left( \prod_{n=0}^{N-1} f_n(y)\right) \left[ \sum_{n=0}^{N-1} \frac{1}{f_n(y)}\right]\PERIOD
%%\end{align}
%%\begin{align}\label{smoothed_integrand_single_opt_1d}
%%	h(\mathbf{z}_{-1})&= \int_{\rset}  g   \left( \Psi \circ \Phi(T;z_1,\mathbf{z}_{-1})\right)   \rho_1(z_1) dz_1.
%%\end{align}
%%\begin{align}\label{eq:resulting_integrand_after_num_smoothing_digital}
%%	h(\mathbf{z}_{-1}) &:=  \int_{\rset} g \left(\Psi \circ \Phi(T;z_1,\mathbf{z}_{-1})\right)   \rho_1(z_1) dz_1 \nonumber\\
%%	&=\int_{-\infty}^{y^\ast} g \left( \Psi \circ \Phi(T;z_1,\mathbf{z}_{-1})\right)  \rho_d(z_1) dz_1 +\int_{y^\ast}^{\infty} g \left( \Psi \circ \Phi(T;z_1,\mathbf{z}_{-1})\right) \rho_d(z_1) dz_1,
%%\end{align}
%%where we use Gauss-Laguerre quadrature with $N_q$ points to approximate each part.

\subsubsection{Single digital option under  the discretized GBM model}\label{sec:Results for the binary option example}
The first example that we test is   the single  digital  option under the discretized GBM model, with   parameters : $T=1$, $\sigma=0.4$ and $S_0=K=100$. The exact reference value of this case is $0.42074$. 

Figure \ref{fig: Comparing the numerical complexity of the different  methods with the different configurations for binary GBM}  shows a comparison of the numerical complexity for each method under the two different scenarios. This Figure shows that, to achieve a relative error below $1\%$, level $1$ of the Richardson extrapolation is the optimal configuration for both the MC and the ASGQ methods.

\begin{figure}[h!]
	\centering % <-- added
	\begin{subfigure}{0.4\textwidth}
		\includegraphics[width=\linewidth]{./figures/Binary_Complexity_rates/error_vs_time_MC_comparison}
		\caption{}
		\label{fig:1}
	\end{subfigure}\hfil % <-- added
	\begin{subfigure}{0.4\textwidth}
		\includegraphics[width=\linewidth]{./figures/Binary_Complexity_rates/error_vs_time_ASGQ_comparison}
		\caption{}
		\label{fig:2}
	\end{subfigure}
	\caption{Digital option under GBM: Comparing the numerical complexity of the different  methods with the different configurations in terms of the level of Richardson extrapolation. CI refers to 95\% confidence intervals. a) MC methods. b) ASGQ methods combined with numerical smoothing.}
	\label{fig: Comparing the numerical complexity of the different  methods with the different configurations for binary GBM}
\end{figure}

We compare these optimal configurations for each method  in Figure \ref{fig:Complexity plot for MC and MISC , Binary}, and we show that  ASGQ  combined with numerical smoothing  outperforms MC in terms of numerical complexity. In particular, to achieve a total relative error around $0.7\%$, ASGQ  combined with numerical smoothing and  level $1$ of Richardson extrapolation requires
approximately $0.7\%$ of the work of MC combined with level $1$ of Richardson extrapolation. 
\FloatBarrier
\begin{figure}[h!]
\centering
\includegraphics[width=0.4\linewidth]{./figures/Binary_Complexity_rates/error_vs_time_full_comparison}
	\caption{Digital option under GBM: Computational work comparison for the different methods with the best configurations, as concluded from Figure \ref{fig: Comparing the numerical complexity of the different  methods with the different configurations for binary GBM}. To achieve a relative error below $1\%$, the ASGQ method combined with numerical smoothing and  level $1$ of Richardson extrapolation significantly outperforms  the  MC  method combined with level $1$ of the Richardson extrapolation. CI refers to 95\% confidence intervals.}
	\label{fig:Complexity plot for MC and MISC , Binary}
\end{figure}
\FloatBarrier
\subsubsection{Single call option under the discretized GBM model}\label{sec:Results for the call option example}
The second  example that we test  is   the single call option under the discretized GBM model, with  parameters: $T=1$, $\sigma=0.4$ and $S_0=K=100$. The exact reference value of this case is $15.8519$. 
 
Figure \ref{fig: Comparing the numerical complexity of the different  methods with the different configurations for call GBM}  shows a comparison of the numerical complexity for each method under the two  scenarios. This Figure shows that, to achieve a relative error of $1\%$, level $1$ of Richardson extrapolation is the optimal configuration for both  methods. 

\begin{figure}[h!]
	\centering % <-- added
	\begin{subfigure}{0.4\textwidth}
		\includegraphics[width=\linewidth]{./figures/Call_Complexity_rates/error_vs_time_MC_comparison}
		\caption{}
		\label{fig:1}
	\end{subfigure}\hfil % <-- added
	\begin{subfigure}{0.4\textwidth}
		\includegraphics[width=\linewidth]{./figures/Call_Complexity_rates/error_vs_time_ASGQ_comparison}
		\caption{}
		\label{fig:2}
	\end{subfigure}
	\caption{Call option under GBM: Comparing the numerical complexity of the different  methods with the different configurations in terms of the level of Richardson extrapolation. CI refers to 95\% confidence intervals. a) MC methods. b) ASGQ methods combined with numerical smoothing.}
	\label{fig: Comparing the numerical complexity of the different  methods with the different configurations for call GBM}
\end{figure}

We compare these optimal configurations for each method  in Figure \ref{fig:Complexity plot for MC and MISC , Call}, and we show that  ASGQ combined with numerical smoothing  outperforms MC in terms of numerical complexity. In particular, to achieve a total relative error around $0.5\%$, ASGQ combined with numerical smoothing and  level $1$ of Richardson extrapolation requires
approximately $0.8\%$ of the work of MC combined with level $1$ of Richardson extrapolation. 
\begin{figure}[h!]
\centering
\includegraphics[width=0.4\linewidth]{./figures/Call_Complexity_rates/error_vs_time_full_comparison}
	\caption{Call option under GBM: Computational work comparison for the different methods with the best configurations, as concluded from Figure \ref{fig: Comparing the numerical complexity of the different  methods with the different configurations for call GBM}. To achieve a relative error below $1\%$, the ASGQ  combined with numerical smoothing and  level $1$ of Richardson extrapolation significantly outperforms  the  MC  method combined with level $1$ of Richardson extrapolation. CI refers to 95\% confidence intervals.}
	\label{fig:Complexity plot for MC and MISC , Call}
\end{figure}

%%	\begin{figure}[h!]
%%	\centering
%%	\includegraphics[width=0.7\linewidth]{./figures/Call_Complexity_rates/error_vs_time_rich}
%%	
%%	\caption{Complexity plot for MC and MISC for the case with Richardson extrapolation.}
%%	\label{fig:Complexity plot for MC and MISC , Call, with rich}
%%\end{figure}
%
%
%
%\begin{figure}[h!]
%	\centering
%	\includegraphics[width=0.4\linewidth]{./figures/Call_Complexity_rates/error_vs_time_comparision}
%	
%	\caption{Complexity plot for MISC without and with Richardson extrapolation, for the call option.}
%	\label{fig:Complexity plot for MC and MISC , Call, comparison}
%\end{figure}
%\FloatBarrier


%%\begin{table}[h!]
%%	\centering
%%	\begin{tabular}{l*{5}{c}r}
%%		Method \textbackslash  Steps    &$1-2-4$        & $2-4-8$ & $4-8-16$   \\
%%		\hline
%%		MISC ($TOL_{\text{MISC}}=5.10^{-1}$)  &$0.0047$ & $  0.0015$ & $0.0019
%%		$   \\
%%		MISC ($TOL_{\text{MISC}}=10^{-3}$) & $ \red{0.0043}$ & $ \red{0.0013}$ & $\red{  0.0017}$    \\
%%		MC method ($M=10^{6}$)&$ \mathbf{0.0041}$    & $\mathbf{0.0013}$  & $\mathbf{0.0016}$  \\
%%		\hline
%%	\end{tabular}
%%	\caption{Relative error of the call option price of the different tolerances for different number of time steps, using Richardson extrapolation (level $2$)}
%%	\label{Relative error of Call option price of the different tolerances for different number of time steps, using Richardson extrapolation (level $2$)}
%%\end{table}

%\begin{figure}[h!]
%	\centering
%	\begin{subfigure}{.35\textwidth}
%		\centering
%		\includegraphics[width=1\linewidth]{./figures/weak_error_rates_call/Beta_10/without_richardson/weak_convergence_order_call_option_relative_M_10_5}
%		\caption{}
%		\label{fig:sub3}
%	\end{subfigure}%
%	\begin{subfigure}{.35\textwidth}
%		\centering
%		\includegraphics[width=1\linewidth]{./figures/weak_error_rates_call/Beta_10/without_richardson/weak_convergence_order_differences_call_option_relative_M_10_5}
%		\caption{}
%		\label{fig:sub4}
%	\end{subfigure}
%	
%	\caption{The rate of convergence of the weak error for the call option, without Richardson extraploation, using MC with $M=10^5$: a) $\abs{\expt{g(X_{\Delta t})}-g(X)}$  b) $\abs{\expt{g(X_{\Delta t})-g(X_{\Delta t/2})}}$ }
%	\label{fig:Weak_rate_call_without_rich}
%\end{figure}
%\begin{figure}[h!]
%	\centering
%	\begin{subfigure}{.35\textwidth}
%		\centering
%		\includegraphics[width=1\linewidth]{./figures/weak_error_rates_call/Beta_10/with_richardson/weak_convergence_order_call_richardson_relative_M_10_6}
%		\caption{}
%		\label{fig:sub3}
%	\end{subfigure}%
%	\begin{subfigure}{.35\textwidth}
%		\centering
%		\includegraphics[width=1\linewidth]{./figures/weak_error_rates_call/Beta_10/with_richardson/weak_convergence_order_differences_call_richardson_relative_M_10_6}
%		\caption{}
%		\label{fig:sub4}
%	\end{subfigure}
%	
%	\caption{The rate of convergence of the weak error for the  call option with Richardson extraploation, using MC with $M=10^6$: a) $\abs{\expt{2 g(X_{\Delta t/2}) -g(X_{\Delta t})}-g(X)}$  b) $\abs{\expt{3 g(X_{\Delta t/2})-g(X_{\Delta t})-2 g(X_{\Delta t/4})}}$ }
%	\label{fig:fig:Weak_rate_call_with_rich}
%\end{figure}



%\begin{figure}[h!]
%	\centering
%	\begin{subfigure}{.4\textwidth}
%		\centering
%		\includegraphics[width=1\linewidth]{./figures/weak_error_rates_call/Beta_10/with_richardson/weak_convergence_order_Call_richardson_level2_relative_M_10_6}
%		\caption{}
%		\label{fig:sub3}
%	\end{subfigure}%
%	\begin{subfigure}{.4\textwidth}
%		\centering
%		\includegraphics[width=1\linewidth]{./figures/weak_error_rates_call/Beta_10/with_richardson/weak_convergence_order_differences_Call_richardson_level2_relative_M_10_6}
%		\caption{}
%		\label{fig:sub4}
%	\end{subfigure}
	
%	\caption{The rate of convergence of the weak error for the  call option with Richardson extraploation (level 2), using MC with $M=10^6$: a) $\abs{\frac{1}{3}\expt{8 g(X_{\Delta t/4}) -6g(X_{\Delta t/2}) +g(X_{\Delta t})}-g(X)}$  b) $\abs{\frac{1}{3}\expt{-8 g(X_{\Delta t/8}) +14g(X_{\Delta t/4})-7 (X_{\Delta t/2}) +g(X_{\Delta t})}}$}
%	\label{fig:Weak_rate_call_with_rich_level2}
%\end{figure}
%\subsubsection*{$\beta=32$}

%\FloatBarrier
%\begin{figure}[h!]
%	\centering
%%	\begin{subfigure}{.35\textwidth}
%%		\centering
%		\includegraphics[width=0.4\linewidth]{./figures/weak_error_rates_call/Beta_32/without_rich/weak_convergence_order_call_option_relative_M_4_10_5}
%%		\caption{}
%%		\label{fig:sub3}
%%	\end{subfigure}%
%%	\begin{subfigure}{.35\textwidth}
%%		\centering
%%		\includegraphics[width=1\linewidth]{./figures/weak_error_rates_call/Beta_32/with_rich/weak_convergence_order_call_richardson_relative}
%%		\caption{}
%%		\label{fig:sub4}
%%	\end{subfigure}
%	
%	\caption{The convergence of the relative weak error  $\mathcal{E}_B(N)$ defined in \ref{eq:total_error}, using MC with $M=4 \times 10^5$ samples  for the call option example. The upper and lower bounds are $95\%$ confidence intervals.}
%	\label{fig:Weak_rate_call_beta_32}
%\end{figure}
%\FloatBarrier

%\begin{figure}[h!]
%	\centering
%	\begin{subfigure}{.35\textwidth}
%		\centering
%		\includegraphics[width=1\linewidth]{./figures/weak_error_rates_call/Beta_32/with_rich/weak_convergence_order_call_richardson_relative}
%		\caption{}
%		\label{fig:sub3}
%	\end{subfigure}%
%	\begin{subfigure}{.35\textwidth}
%		\centering
%		\includegraphics[width=1\linewidth]{./figures/weak_error_rates_call/Beta_32/with_rich/weak_convergence_order_differences_call_richardson_relative}
%		\caption{}
%		\label{fig:sub4}
%	\end{subfigure}
%	
%	\caption{The rate of convergence of the weak error for the  call option with Richardson extraploation (level 1), using MC with $M=5.10^6$: a)   b) $\abs{\expt{3 g(X_{\Delta t/2})-g(X_{\Delta t})-2 g(X_{\Delta t/4})}}$}
%	\label{fig:Weak_rate_call_with_rich_level1_beta_32}
%\end{figure}


%\begin{figure}[h!]
%	\centering
%	\begin{subfigure}{.4\textwidth}
%		\centering
%		\includegraphics[width=1\linewidth]{./figures/weak_error_rates_call/Beta_32/with_rich/weak_convergence_order_Call_richardson_level2_relative_M_5_10_6}
%		\caption{}
%		\label{fig:sub3}
%	\end{subfigure}%
%	\begin{subfigure}{.4\textwidth}
%		\centering
%		\includegraphics[width=1\linewidth]{./figures/weak_error_rates_call/Beta_32/with_rich/weak_convergence_order_differences_Call_richardson_level2_relative_M_5_10_6}
%		\caption{}
%		\label{fig:sub4}
%	\end{subfigure}
%	
%	\caption{The rate of convergence of the weak error for the  call option with Richardson extraploation (level 2), using MC with $M=5.10^6$: a) $\abs{\frac{1}{3}\expt{8 g(X_{\Delta t/4}) -6g(X_{\Delta t/2}) +g(X_{\Delta t})}-g(X)}$  b) $\abs{\frac{1}{3}\expt{-8 g(X_{\Delta t/8}) +14g(X_{\Delta t/4})-7 (X_{\Delta t/2}) +g(X_{\Delta t})}}$}
%	\label{fig:Weak_rate_call_with_rich_level2_beta_32}
%\end{figure}


%\subsubsection{Comparing relative errors}\label{sec:Comparing relative errors, call}
%\subsubsection*{Without Richardson extrapolation}


%
%In this Section, we report the results for the Call option, using the different Methods: MISC, MC $+$ root finding  and MC, without Richardson extrapolation . We mention that for MISC we used a very small tolerance for the Newton solver, when solving the Kink point problem ($TOL_{\text{Newton}}=10^{-10}$), we also used $\beta=32$ (number of Laguerre quadrature points ). We start by reporting the observed approximated values using different methods (See table \ref{table:Call option price of the different methods for different number of time steps, without Richardson extrapolation.}). The biased values for MC method were computed using the values of Bias, reported in table \ref{Bias and Statistical errors of MC  for computing Call option price  for different number of time steps, without Richardson extrapolation. The numbers between parentheses are the corresponding absolute errors.}. In table \ref{Quadrature error of MISC to compute Call option price of the different tolerances for different number of time steps, without Richardson extrapolation. The numbers between parentheses are the corresponding absolute errors.}, we report the behavior of quadrature error with respect to MISC tolerance. We precise that the quadrature error is computed by substracting the MISC approximated value from the biased MC value. We report in red the values where MISC becomes stable (see also figure \ref{fig:Quadrature_error_non_rich_Call}). Those values where used to compute the needed number of samples for MC (with and without root finding), to achieve similar magnitude  for statistical error. Later, in table \ref{Total error of MISC and MC to compute Call option price of the different tolerances for different number of time steps, without Richardson extrapolation. The numbers between parentheses are the corresponding absolute errors.}, we report the total relative error for all methods (Quadrature error + Bias for MISC and Statistical error + Bias for MC). We also report in table \ref{Comparsion of the computational time of  MC and MISC, used to compute Call option price  for different number of time steps, without Richardson extrapolation}, the computational time needed for all different methods.  We finally provide in figure \ref{fig:Complexity plot for MC and MISC , Call non rich}, the complexity rates for the different involved methods.
\subsubsection{Basket call option  under discretized GBM model}\label{sec:The basket call option  under GBM  model}
The third example that we consider under the  GBM  model is the multi-dimensional  basket call option. We consider now  the four dimensional basket call option  with parameters: $\sigma_{1,2,3,4}=0.4$, $\rho=0.3$, $T=1$ $r=0$,  $S_0^{1,2,3,4}=K=100$,  and $c_{1,2,3,4}=1/4$. The reference value for those parameters  is  $11.04$. Our experiments show that Richardson extrapolation did not improve the performance of both considered methods, and  figure \ref{fig:Complexity plot for MC and MISC , 4 dim basket call non rich} shows that ASGQ combined with numerical smoothing  requires approximately $7\%$ of the work of MC  to achieve a total relative error of around $0.8\%$.
%\FloatBarrier
	\begin{figure}[h!]
\centering
\includegraphics[width=0.4\linewidth]{./figures/basket_call_4d_time_stepping/complexity_rates/error_vs_time}

\caption{$4$-dimensional basket call option under GBM: Computational work comparison for the different methods. To achieve a relative error below $1\%$, ASGQ  combined with numerical smoothing significantly outperforms the  MC method. CI refers to 95\% confidence intervals.}
\label{fig:Complexity plot for MC and MISC , 4 dim basket call non rich}
\end{figure}

%\FloatBarrier

%Figure \ref{fig:Weak_rate_4_dim_basket} shows the estimated   weak error  for the case without Richardson extrapolation, and we report 

%\FloatBarrier
%\begin{figure}[h!]
%		\centering
%		\includegraphics[width=0.4\linewidth]{./figures/basket_call_4d_time_stepping/weak_convergence/weak_convergence_order_basket_option_4d_relative_M_4_10_6_beta_256}
%
%	\caption{The convergence of the relative weak error  $\mathcal{E}_B(N)$ defined in \ref{eq:total_error}, for the $4$-dimensional basket call option with  a number of Laguerre  quadrature points  $\beta=512$ and number of samples for MC $M=4 \times 10^6$. The upper and lower bounds are $95\%$ confidence intervals.}
%	\label{fig:Weak_rate_4_dim_basket}
%\end{figure}


%\subsection{The call on max  option under GBM}\label{sec:The best call option  under GBM}
%The fourth example that we consider is  the European rainbow option under BBM model and in particular the call on max option whose payoff is given by
%\begin{align}\label{eq:max_call_option}
%\max\left( \max\left(S_1,\dots,S_d\right)-K,0 \right).
%\end{align}
%
%We start here by the two dimensional call on max option under the GBM model. The discretization of the assets is the same as given in  \eqref{eq:discrete_rep_2} and \eqref{eq: incremental functions}, where we use the same transformation as in Section \ref{sec:Step $1$: Numerical smoothing}. This implies that, in order to determine $Y^{\ast}_1$, we need to solve
%\begin{align}
%	x=\max\left(X_0^{(1)}  \prod_{i=0}^{N-1} g_i^{(1)}(Y^{\ast}_1(x),\mathbf{Y}_{-1}),X_0^{(2)}  \prod_{i=0}^{N-1} g_i^{(2)}(Y^{\ast}_1(x),\mathbf{Y}_{-1})\right)
%\end{align}
%
%
%For illustration, we consider the example with parameters:  $S_0^{1,2}=K=100$, $\sigma_{1,2}=0.4$, $\rho=0.3$, $T=1$, and  $r=0$, the reference value for those parameters  is  $26.40$.


%\subsubsection*{$d=2$}
%For illustration, we start with the two dimensional basket call option  with parameters:  $S_0^{1,2}=K=100$, $\sigma_{1,2}=0.4$, $\rho=0.3$, $T=1$ $r=0$ and $c_{1,2}=1/2$, the reference value for those parameters  is  $12.90$. Figure \ref{fig:Weak_rate_two_dim_basket} shows the estimated   weak error  for the case without Richardson extrapolation, and we report the results for comparing MC and ASGQ in Tables \ref{Total error of MISC and MC to compute two  dim basket  Call option price of the different tolerances for different number of time steps, without Richardson extrapolation. The numbers between parentheses are the corresponding absolute errors.} and \ref{Comparsion of the computational time of  MC and MISC, used to compute two dim basket Call option price  for different number of time steps, without Richardson extrapolation}, and Figure \ref{fig:Complexity plot for MC and MISC , two dim basket call non rich}. Our numerical experiments show that ASGQ  requires approximately $5\%$ of the work of MC  to achieve a total relative error of around $0.9\%$.
%
%\FloatBarrier
%\begin{figure}[h!]
%		\centering
%		\includegraphics[width=0.4\linewidth]{./figures/basket_call_2d_time_stepping/weak_convergence/weak_convergence_order_basket_option_2d_relative_M_10_7_beta_128}
%
%	\caption{The convergence of the relative weak error  $\mathcal{E}_B(N)$ defined in \ref{eq:total_error}, for the two dimensional basket call option with  a number of Laguerre  quadrature points  $\beta=128$ and number of samples for MC $M=10^7$. The upper and lower bounds are $95\%$ confidence intervals.}
%	\label{fig:Weak_rate_two_dim_basket}
%\end{figure}
%\FloatBarrier
%
%
%\FloatBarrier
%\begin{table}[h!]
%	\centering
%	\begin{tabular}{l*{6}{c}r}
%		\toprule[1.5pt]
%	Method & & Steps  & &     \\
%	\hline
%           & $2$ & $4$ & $8$   \\
%		\hline
%		ASGQ   &  $\underset{(0.01,0.006)}{\mathbf{0.016}}$ & $\underset{(0.0079,0.0055)}{\mathbf{0.0134}}$ & $\underset{(0.0043,0.0042)}{\mathbf{0.0085}}$   \\
%
%		\hline		
%			MC +root finding   &  $\underset{(0.01,0.01)}{\mathbf{0.02}}$ & $\underset{(0.0079,0.0076)}{\mathbf{0.0155}}$ & $\underset{(0.0043,0.0038)}{\mathbf{0.0081}}$  \\
%			M(\# MC samples)   & $2 \times 10^3$   &  $5 \times 10^3$ & $2 \times 10^4$  \\	
%		\hline	
%				MC   &  $\underset{(0.01,0.01)}{\mathbf{0.02}}$ & $\underset{(0.0079,0.0076)}{\mathbf{0.0155}}$ & $\underset{(0.0043,0.004)}{\mathbf{0.0083}}$   \\	
%				M(\# MC samples)   &$10^5$  & $2 \times 10^5$  &  $8 \times 10^5$\\	
%		
%			\bottomrule[1.25pt]
%	\end{tabular}
%	\caption{Total relative  error of ASGQ, with different tolerances, and MC to compute two dimensional basket call option price for different number of time steps, without Richardson extrapolation. The values between parentheses correspond to the different errors contributing to the total relative error: for ASGQ we report the bias and quadrature errors and for MC we report the bias and the statistical errors. The number of MC samples,$ M$, is chosen to satisfy \eqref{optimal_number_samples}.}
%	\label{Total error of MISC and MC to compute two  dim basket  Call option price of the different tolerances for different number of time steps, without Richardson extrapolation. The numbers between parentheses are the corresponding absolute errors.}
%\end{table}
%\FloatBarrier
%
%
%
%
%\begin{table}[h!]
%	\centering
%	\begin{tabular}{l*{6}{c}r}
%		\toprule[1.5pt]
%	Method & & Steps  & &     \\
%	\hline
%	         & $2$ & $4$ & $8$    \\
%		\hline
%		ASGQ & $4$  & $8$ & $21$     \\
%			MC +root finding  & $281$&  $814$&  $3888$   \\
%				MC  &   $34$& $93$ &   $ 442$ \\
%		\bottomrule[1.25pt]
%	\end{tabular}
%	\caption{Comparison of the computational time of  MC and ASGQ, used to compute two dimensional basket call option price  for different number of time steps, without Richardson extrapolation. The average computational time of MC is computed over $10$ runs.}
%	\label{Comparsion of the computational time of  MC and MISC, used to compute two dim basket Call option price  for different number of time steps, without Richardson extrapolation}
%\end{table}
%
%
%\FloatBarrier
%	\begin{figure}[h!]
%\centering
%\includegraphics[width=0.4\linewidth]{./figures/basket_call_2d_time_stepping/complexity_rates/error_vs_time}
%
%\caption{Computational work comparison for ASGQ and MC methods, for the case of two dimensional basket call option. This plot shows that to achieve a relative error below $1\%$, ASGQ outperforms significantly MC method in terms of computational time.}
%\label{fig:Complexity plot for MC and MISC , two dim basket call non rich}
%\end{figure}
%
%
%\FloatBarrier
%
%\subsubsection*{$d=4$}
\subsection{Options  under the discretized  Heston model}\label{sec:options  under the discretized  Heston model}
In this section, we consider  testing options under the discretized Heston model \cite{heston1993closed,broadie2006exact,kahl2006fast,andersen2007efficient} whose dynamics are given by
\begin{small}
\begin{align}\label{eq:dynamics Heston}
dS_t&=\mu S_t dt+\sqrt{v_t}S_t dW_t^S= \mu S_t dt+ \rho\sqrt{v_t}S_t dW_t^v+ \sqrt{1-\rho^2} \sqrt{v_t}S_t dW_t \nonumber\\
dv_t&=\kappa (\theta-v_t)dt+\xi \sqrt{v_t} dW_t^v\COMMA
\end{align}\end{small}
where 
$S_t$ is the price of the asset; $v_t$ is the instantaneous variance, given as  a CIR process; $\left(W_{t}^{S},W_{t}^{v}\right)$ are correlated Wiener processes with correlation $\rho$; $\mu$  is the rate of return of the asset; $\theta$ is  the mean  variance; $\kappa$ is the rate at which $v_t$ reverts to $\theta$; and $\xi$ is the volatility of the volatility.

Given that the SDE for the asset path is now dependent  upon the solution of the  volatility SDE in \eqref{eq:dynamics Heston}, we must simulate the volatility process first and then use it to simulate the asset path.  Therefore, a numerical approximation (discretization)  is needed to obtain both paths. To this end, many simulation schemes have been proposed in the literature.   In Appendix \ref{sec:Schemes to simulate the Heston dynamics}, we  give an overview of the most popular  methods in this context. These methods mainly differ in the way they simulate the volatility process to ensure its positiveness.

Note that we are using ASGQ, which is very sensitive to the smoothness of the integrand. We found numerically (see section \ref{sec:On the choice of the simulation scheme of the Heston model}) that using a non-smooth transformation to ensure the positiveness of the volatility process deteriorates the performance of the ASGQ. We suggest an alternative way  in this work, to guarantee the positiveness of the volatility process,  to simulate it as  the sum of  Ornstein-Uhlenbeck (OU) or Bessel processes as suggested in Appendix \ref{sec:Discretization of Heston model with the volatility process Simulated using the sum of  Ornstein-Uhlenbeck (Bessel) processes}.

In the literature  \cite{andersen2007efficient, lord2010comparison,alfonsi2010high}, more focus was on designing schemes that i) ensures the positiveness  of the volatility process and ii) has a good weak error behavior. In our setting, an optimal scheme is defined through two properties: i) the behavior of mixed differences rates, which is an important feature for an  optimal performance of ASGQ (see  Appendix \ref{sec:Comparison in terms of  the weak error behavior} for more details), and  ii) the behavior of the weak error in order to apply the Richardson extrapolation when it is needed. We refer to Appendices \ref{sec:Comparison in terms of mixed differences rates} and \ref{sec:Comparison in terms of  the weak error behavior} for more details on the comparison of the different schemes, which suggest that  the Heston OU-based scheme,  defined in Section \ref{sec:Discretization of Heston model with the volatility process Simulated using the sum of  Ornstein-Uhlenbeck (Bessel) processes},  gives the best results according to our criteria.   Therefore, in our numerical experiments, we use this scheme with the ASGQ method. For the MC method, we use the full truncation scheme,  as explained in Section \ref{sec:Discretization of Heston model with a non smooth transformations for the volatility process}.
\begin{remark}
Although we compare different simulation schemes for the Heston model, to ensure a sub-optimal performance of the ASGQ combined with numerical smoothing,  we emphasize that we do not claim that the chosen scheme is the optimal scheme for all parameters constellations, and a more thorough study on this topic is left as a future work. In this work, we instead aim at highlighting the advantage of our numerical smoothing idea.
\end{remark}
\begin{remark}
Although we only illustrate the numerical results for one set of  parameters for the Heston model, we note that  we obtained  almost similar results for  many other cases.
\end{remark}

\subsubsection{Digital option  under the discretized  Heston model}\label{sec:Digital option under the discretized  Heston model with parameters of Set 1}
We consider   the  digital option  under the discretized  Heston model  with parameters: $S_0=K=100$, $v_0=0.04$, $\mu=0$,  $\rho=-0.9$, $\kappa=1$, $\xi=0.1$, $\theta=0.0025$. The reference solution  is   $0.5145$. 

Figure \ref{fig: Comparing the numerical complexity of the different  methods with the different configurations for digital Heston}  shows a comparison of the numerical complexity for each method under the two different scenarios. From this figure, we can conclude that, to achieve a relative error of $1\%$, level $1$ of Richardson extrapolation is the optimal configuration for  the ASGQ method, and without Richardson extrapolation is the optimal configuration for  the MC method. 
%\FloatBarrier
\begin{figure}[h!]
	\centering % <-- added
	\begin{subfigure}{0.4\textwidth}
		\includegraphics[width=\linewidth]{./figures/Heston_digital/complexity_MISC_MC/error_vs_time_MC_comparison}
		\caption{}
		\label{fig:1}
	\end{subfigure}\hfil % <-- added
	\begin{subfigure}{0.4\textwidth}
		\includegraphics[width=\linewidth]{./figures/Heston_digital/complexity_MISC_MC/error_vs_time_ASGQ_comparison}
		\caption{}
		\label{fig:2}
	\end{subfigure}
	\caption{Digital option under Heston: Comparing the numerical complexity of the different  methods with the different configurations in terms of the level of Richardson extrapolation. CI refers to 95\% confidence intervals. a) MC methods. b) ASGQ methods combined with numerical smoothing.}
	\label{fig: Comparing the numerical complexity of the different  methods with the different configurations for digital Heston}
\end{figure}

We compare these optimal configurations for each method  in Figure \ref{fig:Complexity plot for MC and MISC , digital Heston}, which  shows that,  to achieve a total relative error around $0.6\%$, ASGQ  combined with numerical smoothing and  level $1$ of Richardson extrapolation requires
approximately $6\%$ of the work of MC  without Richardson extrapolation. 
\FloatBarrier
\begin{figure}[h!]
\centering
\includegraphics[width=0.4\linewidth]{./figures/Heston_digital/complexity_MISC_MC/error_vs_time_full_comparison}
	\caption{Digital option under Heston: Computational work comparison for the different methods with the best configurations, as concluded from Figure \ref{fig: Comparing the numerical complexity of the different  methods with the different configurations for digital Heston}. To achieve a relative error below $1\%$, the ASGQ combined with numerical smoothing and  level $1$ of Richardson extrapolation significantly outperforms   the  MC  method without the Richardson extrapolation. CI refers to 95\% confidence intervals.}
	\label{fig:Complexity plot for MC and MISC , digital Heston}
\end{figure}
\FloatBarrier

\subsubsection{European call option  under the discretized  Heston model}\label{sec:European call option  under the discretized  Heston model with parameters of Set 1}
We consider   the  call option  under the discretized  Heston model  with parameters: $S_0=K=100$, $v_0=0.04$, $\mu=0$,  $\rho=-0.9$, $\kappa=1$, $\xi=0.1$, $\theta=0.0025$. The reference solution is   $6.332542$.

Figure \ref{fig: Comparing the numerical complexity of the different  methods with the different configurations for call Heston}  shows a comparison of the numerical complexity for each method under the two different scenarios. From this Figure, we conclude that level $1$ of Richardson extrapolation is the optimal configuration for both the MC and the ASGQ methods. 
\FloatBarrier
\begin{figure}[h!]
	\centering % <-- added
	\begin{subfigure}{0.4\textwidth}
		\includegraphics[width=\linewidth]{./figures/Heston_single_call_smooth_vol/complexity_rates/set1/error_vs_time_MC_comparison}
		\caption{}
		\label{fig:1}
	\end{subfigure}\hfil % <-- added
	\begin{subfigure}{0.4\textwidth}
		\includegraphics[width=\linewidth]{./figures/Heston_single_call_smooth_vol/complexity_rates/set1/error_vs_time_ASGQ_comparison}
		\caption{}
		\label{fig:2}
	\end{subfigure}
	\caption{Call option under Heston: Comparing the numerical complexity of the different  methods with the different configurations in terms of the level of Richardson extrapolation. CI refers to 95\% confidence intervals. a) MC methods. b) ASGQ methods combined with numerical smoothing.}
	\label{fig: Comparing the numerical complexity of the different  methods with the different configurations for call Heston}
\end{figure}
\FloatBarrier
We compare these optimal configurations for each method  in Figure \ref{fig:Complexity plot for MC and MISC , Call Heston}, which  shows that  ASGQ  outperforms MC in terms of numerical complexity. In particular, to achieve a total relative error around $0.5\%$, ASGQ combined with numerical smoothing and  level $1$ of Richardson extrapolation requires
approximately $17\%$ of the work of MC combined with level $1$ of Richardson extrapolation.
\FloatBarrier 
\begin{figure}[h!]
\centering
\includegraphics[width=0.4\linewidth]{./figures/Heston_single_call_smooth_vol/complexity_rates/set1/error_vs_time_full_comparison}
	\caption{Call option under Heston: Computational work comparison for the different methods with the best configurations, as concluded from Figure \ref{fig: Comparing the numerical complexity of the different  methods with the different configurations for call Heston}. To achieve a relative error below $1\%$, the ASGQ combined with numerical smoothing and  level $1$ of Richardson extrapolation significantly outperforms   the  MC  method combined with level $1$ of Richardson extrapolation. CI refers to 95\% confidence intervals.}
	\label{fig:Complexity plot for MC and MISC , Call Heston}
\end{figure}
\FloatBarrier




==> Setting.tex <==
%In the context of option pricing, we aim at approximating the option price, $E[g(\mathbf{X}(t))]$,  where $g:\mathbb{R}^d  \rightarrow \mathbb{R}$ is the payoff function  and where  the process of the asset prices $\mathbf{X} \in \mathbb{R}^d$ solves 
%\begin{align*}
%	\mathbf{X}(t)=\mathbf{X}(0)+ \int_{0}^{t} a(s,\mathbf{X}(s)) ds + \sum_{\ell=1}^{\ell_0} \int_{0}^{t} b^{\ell}(s,\mathbf{X}(s)) dW^{\ell}(s)
%\end{align*}
%Let us denote  by $\Phi: (\mathbf{z}_1,\dots,\mathbf{z}_N) \rightarrow \bar{\mathbf{X}}_T$, the mapping consisting of the time-stepping scheme, where $\{\mathbf{z}_i\}_{i=1}^N$ are independent $d$-dimensional Gaussian random vectors, and $N$ is the number of time steps. Without loss of Generality, we assume that $\Phi$ may include pre-processing transformations to reduce the effective dimension. We also assume that $d=1$ and the extension to higher dimension is trivial.
%
%In this setting, we are interetsed in the basic problem of approximating
%\begin{align}\label{eq:multivariate integral}
%E[g(\mathbf{X}(T))] &\approx E[g(\bar{\mathbf{X}}_T)] \nonumber\\
%&=\int_{\rset^N}g \circ \Phi(\mathbf{z})	d \mathbf{z}= \int_{-\infty}^{\infty} \dots \int_{-\infty}^{\infty} g \circ \Phi(z_1,\dots,z_N) \rho_d(\mathbf{z}) dz_1,\dots,dz_N \nonumber\\
%&=I_N (g \circ \Phi) \COMMA
%\end{align}
%with
%\begin{equation*}\label{eq: multivariate gaussian distribution}
%\rho_N(\mathbf{z})=\frac{1}{(2 \pi)^{N/2}} e^{-\frac{1}{2} \mathbf{z}^T \mathbf{z}} \PERIOD
%\end{equation*} 
%where $\rho$ is a continuous and strictly positive probability density function on $\rset$ and $g$ is a real-valued function integrable with respect to $\rho_N$.
 



==> abstract.tex <==

\

\textbf{Keywords} .

\textbf{2010 Mathematics Subject Classification} .

==> commands.tex <==
%%%%%%%%%%%%
% commands %
%%%%%%%%%%%%

%packages
\usepackage[leqno]{amsmath}
\usepackage{amsthm}
\usepackage{bbm}
\usepackage{enumerate}
\usepackage[round,longnamesfirst]{natbib}
\usepackage[bookmarksopen,pdfstartview=FitH]{hyperref}
\hypersetup{colorlinks,%
            citecolor=blue,%
            filecolor=blue,%
            linkcolor=blue,%
            urlcolor=blue}%
\usepackage{dsfont}
\usepackage{mathtools}
\usepackage[mathscr]{euscript}
\usepackage{nicefrac,booktabs,mathrsfs}
\usepackage{nth}
\usepackage[dvipsnames]{xcolor}
%\usepackage[color]{showkeys}
\definecolor{refkey}{gray}{0.5}
\definecolor{labelkey}{gray}{.7}
\usepackage[backgroundcolor=white,bordercolor=orange]{todonotes}
\usepackage{upgreek}
\usepackage[dvipsnames]{xcolor}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{amssymb}
\usepackage[mathscr]{euscript}
\usepackage{xspace}
\usepackage{epsfig,rotating}
\usepackage{graphicx}
\input{xy}\xyoption{all}

\usepackage{lscape}
\usepackage{enumitem}
\usepackage{upgreek}
\usepackage{subfigure} 
\usepackage{epstopdf}

% \usepackage{txgreeks}
% \usepackage[T1]{fontenc}

\usepackage[left=1.10in,right=1.10in,top=1.40in,bottom=1.30in]{geometry}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\DeclareMathAlphabet{\mathpzc}{OT1}{pzc}{m}{it}


%%%%%%%%%%%%%

%Textstyles


%letters 
\renewcommand{\P}{\mathbb{P}} %probability
\newcommand{\E}{\mathbb{E}} %expectation
\newcommand{\FF}{\mathbb{F}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cD}{\mathcal{D}}


%common math symbols
\def\half{\frac1{2}}
\newcommand{\ind}{\mathbbm1}

%other symbold, common names
\newcommand{\cadlag}{c{\'a}dl{\'a}g }
\newcommand{\Levy}{L{\'e}vy }


%common math notation
\newcommand{\cond}[1]{\left.#1\right\vert}%to get a vert with the right size

%brackets
\newcommand{\brac}[1]{\ensuremath{\left(#1\right)}}
\newcommand{\Brac}[1]{\ensuremath{\big(#1\big)}}
\newcommand{\BRac}[1]{\ensuremath{\Big(#1\Big)}}
\newcommand{\BRAc}[1]{\ensuremath{\bigg(#1\bigg)}}
\newcommand{\BRAC}[1]{\ensuremath{\Bigg(#1\Bigg)}}

\newcommand{\brak}[1]{\ensuremath{\left[#1\right]}}
\newcommand{\scal}[1]{\ensuremath{\left\langle#1\right\rangle}}
\newcommand{\set}[1]{\ensuremath{\left\{#1\right\}}}
\newcommand{\Norm}[1]{\left\Vert#1\right\Vert}%doudle vert norm
\newcommand{\norm}[1]{\left\vert#1\right\vert}%single vert norm




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%% ========================================================================== %%
%% ========================================================================== %%

\theoremstyle{plain}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem*{proposition*}{Proposition}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{axiom}{Axiom}
\newtheorem{hypothesis}[theorem]{Hypothesis}  %[section]



\theoremstyle{definition*}
\newtheorem{example*}{Example}
\theoremstyle{definition}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{note}{Note}[section]
\newtheorem{definition}[theorem]{Definition}
\newtheorem{example}[theorem]{Example}
\newtheorem*{ackn}{Acknowledgements}
\newtheorem{assumption}{Assumption}
\newtheorem{approach}{Approach}
\newtheorem{critique}{Critique}
\newtheorem{question}{Question}
\newtheorem{aim}{Aim}
\newtheorem*{assucd}{Assumption ($\mathbb{CD}$)}
\newtheorem*{asa}{Assumption ($\mathbb{A}$)}
\newtheorem*{appS}{Approximation ($\mathbb{S}$)}
\newtheorem*{appBS}{Approximation ($\mathbb{BS}$)}
% \newtheorem*{asp}{Assumption ($\P$)}
% \newtheorem*{ass}{Assumption ($\mathbb{S}$)}
%% 


%% ========================================================================== %%
\renewcommand{\theequation}{\thesection.\arabic{equation}}
\numberwithin{equation}{section}

\renewcommand{\thefigure}{\thesection.\arabic{figure}}
\numberwithin{equation}{section}

\newcommand{\Law}{\ensuremath{\mathop{\mathrm{Law}}}}
\newcommand{\loc}{{\mathrm{loc}}}

\let\SETMINUS\setminus
\renewcommand{\setminus}{\backslash}

\def\stackrelboth#1#2#3{\mathrel{\mathop{#2}\limits^{#1}_{#3}}}

% \makeatletter
% \def\Ddots{\mathinner{\mkern1mu\raise\p@
% \vbox{\kern7\p@\hbox{.}}\mkern2mu
% \raise4\p@\hbox{.}\mkern2mu\raise7\p@\hbox{.}\mkern1mu}}
% \makeatother
% 
% \newcommand\llambda{{\mathchoice
%      {\lambda\mkern-4.5mu{\raisebox{.4ex}{\scriptsize$\backslash$}}}
%      {\lambda\mkern-4.83mu{\raisebox{.4ex}{\scriptsize$\backslash$}}}
%      {\lambda\mkern-4.5mu{\raisebox{.2ex}
% {\footnotesize$\scriptscriptstyle\backslash$}}}
%      {\lambda\mkern-5.0mu{\raisebox{.2ex}
% {\tiny$\scriptscriptstyle\backslash$}}}}}

\newcommand{\prozess}[1][L]{{\ensuremath{#1=(#1_t)_{t\in[0,T]}}}\xspace}
\newcommand{\prazess}[1][L]{{\ensuremath{#1=(#1_t)_{t\ge0}}}\xspace}
\newcommand{\pt}[1][N]{\ensuremath{\P_{#1}}\xspace}
\newcommand{\tk}[1][N]{\ensuremath{T_{#1}}\xspace}
\newcommand{\dd}[1][]{\ensuremath{\ud{#1}}\xspace}


\newcommand{\bscal}[2]{\ensuremath{\big\langle #1, #2 \big\rangle}}

%\newcommand{\R}[1][\R]{\ensuremath{\R^{#1}}\xspace}
% \newcommand{\pt}[1][]{{\ensuremath{\P_{T^*_{#1}}}}\xspace}
% \newcommand{\ts}[1][]{\ensuremath{T^*_{#1}}\xspace}
%% ========================================================================== %%
%% ========================================================================== %%
\def\lev{L\'{e}vy\xspace}
\def\lk{L\'{e}vy--Khintchine\xspace}
\def\lib{LIBOR\xspace}
\def\mg{martingale\xspace}
\def\smmg{semimartingale\xspace}
\def\alm{affine LIBOR model\xspace}
\def\alms{affine LIBOR models\xspace}
\def\dalms{defaultable \alms}
\def\ap{affine process\xspace}
\def\aps{affine processes\xspace}

\def\half{\frac1{2}}

\def\F{\ensuremath{\mathcal{F}}}
\def\bD{\mathbf{D}}
\def\bF{\mathbf{F}}
\def\bG{\mathbf{G}}
\def\bH{\mathbf{H}}
\def\R{\ensuremath{\mathbb{R}}}
\def\Rp{\mathbb{R}_{\geqslant0}}
\def\Rm{\mathbb{R}_{\leqslant 0}}
\def\C{\ensuremath{\mathbb{C}}}
\def\U{\ensuremath{\mathcal{U}}}
\def\I{\mathcal{I}}
\def\N{\mathbbN}

\def\P{\ensuremath{\mathbb P}} %{\ensuremath{\mathrm{I\kern-.2em P}}}
%\def\Q{\ensuremath{\mathrm{I\kern-.2em Q}}} % looks strange?
\def\Q{\mathbb{Q}}
\def\E{\ensuremath{\mathbb E}} %{\ensuremath{\mathrm{I\kern-.2em E}}}

\def\hP{\ensuremath{\widehat{\mathrm{I\kern-.2em P}}}}
\def\hE{\ensuremath{\widehat{\mathrm{I\kern-.2em E}}}}

\def\bP{\ensuremath{\overline{\mathrm{I\kern-.2em P}}}}
\def\bE{\ensuremath{\overline{\mathrm{I\kern-.2em E}}}}

\def\bphi{\overline{\phi}}
\def\bpsi{\overline{\psi}}

\def\ott{{0\leq t\leq T}}
\def\idd{{1\le i\le d}}

\def\icc{\mathpzc{i}}
\def\ecc{\mathbf{e}_\mathpzc{i}}

\def\uk{u_{k+1}}
\def\vk{v_{k+1}}

\def\e{\mathrm{e}}
\def\a{\mathrm{a}}
\def\b{\mathrm{b}}
\def\ud{\ensuremath{\mathrm{d}}}
\def\dt{\ud t}
\def\dr{\ud r}
\def\ds{\ud s}
\def\dx{\ud x}
\def\dy{\ud y}
\def\dv{\ud v}
\def\du{\ud u}
\def\dw{\ud w}
\def\dz{\ud z}
\def\dsdx{\ensuremath{(\ud s, \ud x)}}
\def\dtdx{\ensuremath{(\ud t, \ud x)}}

\def\rx{\mathrm{x}}

\def\1{\boldsymbol1}
\def\i{\mathrm{i}}
\def\wf{\widehat f}

\def\tc{\ensuremath{\mathpzc{T}}}
\def\afflm{\ensuremath{(X,\mathcal{X},T_N,u,v)}\xspace}

\def\lsnc{\ensuremath{\mathrm{LSNC-}\chi^2}}
\def\nc{\ensuremath{\mathrm{NC-}\chi^2}}


%% ========================================================================== %%
%% ========================================================================== %%

\newcommand{\cG}{{\mathcal{G}}}
\newcommand{\cH}{{\mathcal{H}}}
\newcommand{\cK}{{\mathcal{K}}}
\newcommand{\cM}{{\mathcal{M}}}
\newcommand{\cT}{{\mathcal{T}}}
\newcommand{\ha}{{\mathbb{H}}}
\newcommand{\indik}{{\mathbf1}}
\newcommand{\ifdefault}[1]{\ensuremath{\mathbf1_{\{\tau \leq #1\}}}}
\newcommand{\ifnodefault}[1]{\ensuremath{\mathbf1_{\{\tau > #1\}}}}

\newcommand\bovermat[2]{%
	\makebox[0pt][l]{$\smash{\overbrace{\phantom{%
					\begin{matrix}#2\end{matrix}}}^{#1}}$}#2}
\newcommand\bundermat[2]{%
	\makebox[0pt][l]{$\smash{\underbrace{\phantom{%
					\begin{matrix}#2\end{matrix}}}_{#1}}$}#2}
\makeatletter



\newcommand{\robert}[1]{\todo[linecolor=blue!40!white,backgroundcolor=blue!20!white,size=\footnotesize]{Robert: #1}}

\def\red{\color{red}}
\def\blue{\color{magenta}}
\def\green{\color{OliveGreen}}

\newcommand{\rr}[1]{{\red #1}}
\newcommand{\rg}[1]{{\green #1}}
%% ========================================================================== %%
%% ========================================================================== %%
\newcommand{\abs}[1]{\left\lvert #1 \right\rvert}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%chiheb commands

\newcommand{\ie}{\emph{i.e.}}
\newcommand{\eg}{\emph{e.g.}}
\newcommand{\cf}{\emph{cf.}}
\newcommand{\prob}[1]{\mathrm{P}\left(#1\right)}
\newcommand{\expt}[1]{\mathrm{E}\left[#1\right]}
\newcommand{\expth}[1]{\hat{\mathrm{E}}\left[#1\right]}
\newcommand{\var}[1]{\mathrm{Var}\left[#1\right]}


\newcommand{\rset}{\mathbb{R}}
\newcommand{\nset}{\mathbb{N}}
\newcommand{\zset}{\mathbb{Z}}

\newcommand{\PERIOD}{.}
\newcommand{\COMMA}{,}
\newcommand{\BIGSPACE}{\,\,\,\,\,\,\,}



\newcommand{\Ordo}[1]{{\mathcal{O}}\left(#1\right)}
\newcommand{\ordo}[1]{{o}\left(#1\right)}

==> path_generation_method.tex <==
\subsection{Path generation methods (PGM)}\label{sec:Path generation methods (PGM)}

In the literature of adaptive sparse grids and  QMC, several hierarchical path generation methods (PGMs) or transformation methods have been proposed to reduce the effective dimension. Among these transformations, we cite the Brownian bridge (Bb)  construction \cite{moskowitz1996smoothness,caflisch1997valuation,morokoff1998generating,larcher2003tractability}, the principal component analysis (PCA)  \cite{acworth1998comparison} and the linear transformation (LT) \cite{imai2004minimizing}, etc \dots 

Assume that one wants to compute $\expt{g(B)}$, where $B$ is a Brownian motion with index set $[0,T]$. In most applications this is can be reasonably approximated by $\expt{\tilde{g}\left(B_{\frac{T}{N}}, \dots, B_{\frac{T N}{N}}  \right)}$, where $\tilde{g}$ is a function of the set of discrete Brownian paths.

There are three classical methods for sampling from $\left(B_{\frac{T}{N}}, \dots, B_{\frac{T N}{N}}  \right)$ given a standard normal vector $Z$, namely the forward method, the Brownian bridge (Bb) construction and the principal component analysis (PCA) construction. All of these constructions may be written in the form $\left(B_{\frac{T}{N}}, \dots, B_{\frac{T N}{N}}  \right)=AZ$, where $A$ is an $N \times N$ real matrix with 

\begin{equation}\label{eq:covariance_matrix_in_time}
A A^T =\Sigma:= \left(\frac{T}{N} \min(j,k)\right)_{j,k=1}^N=\frac{T}{N} \begin{bmatrix}
	1       & 1 & 1 & \dots & 1\\
	1     & 2 & 2 & \dots & 2 \\
	1     & 2& 3 & \dots &3 \\
	\vdots    & \vdots& \vdots & \ddots &\vdots \\
	1      & 2 & 3 & \dots &N
\end{bmatrix}
\PERIOD
\end{equation}   
For instance, the matrix $A$ corresponding to the forward method is given by 
\begin{equation*}
	A^{F} = \sqrt{\frac{T}{N}}  \begin{bmatrix}
		1       & 0  & \dots & 0\\
		1     & 1  & \dots & 0 \\
		\vdots    & \vdots & \ddots &\vdots \\
		1      & 1&  \dots &1
	\end{bmatrix}
	\PERIOD
\end{equation*}  
In the case of Bb construction, details about the construction are given in Section \ref{sec:Brwonian bridge construction}, and  the corresponding matrix $A$, For $N=8$ is given by 
 \begin{equation*}
 	A^{\text{Bb}} = \sqrt{T}  \begin{bmatrix}
 		\frac{1}{8}       & 	\frac{1}{8}   & 	\frac{\sqrt{2}}{8} & 0 &\frac{2}{8}  & 0 &0 & 0\\
 	\frac{2}{8}       & 	\frac{2}{8}   & 	\sqrt{2}\frac{ 2}{8} & 0 &0 & 0 &0 & 0\\
 		\frac{3}{8}       & 	\frac{3}{8}   & 	\frac{\sqrt{2}}{8} & 0 &0 &\frac{2}{8} &0  &0 \\
 		 	\frac{4}{8}       & 	\frac{4}{8}   & 	0 & 0 &0 & 0 &0 & 0\\
 		 	\frac{5}{8}       & 	\frac{3}{8}   & 	0 & \frac{\sqrt{2}}{8} &0 &0 &\frac{2}{8} &0 \\
 		 		\frac{6}{8}       & 	\frac{2}{8}   & 	0 & \sqrt{2}\frac{ 2}{8}  &0 & 0 &0 & 0\\
 		 			\frac{7}{8}       & 	\frac{1}{8}   & 	0 & \frac{\sqrt{2}}{8} &0 &0 &0 &\frac{2}{8}  \\
 		 			1       & 0  & 	0 & 0 &0 &0 &0 &0 \\
 	
 	\end{bmatrix}
 	\PERIOD
 \end{equation*}
When doing PCA construction \cite{acworth1998comparison}, we have $A^{\text{PCA}}=VD$, where $\Sigma=V D^2V^T$ is the singular value decomposition of $\Sigma$. 

\subsubsection{More details on Bb}

Describing construction \ref{eq:BB construction}: we  first generate the final value $B_T$, then sample $B_{T/2}$ conditional
on the values of $B_T$ and $B_0$, and proceed by progressively filling in intermediate values. Bb uses the first several coordinates of the low-discrepancy points to determine the general shape of the Brownian path, and the last few coordinates influence only the fine detail of the path. Therefore, the most important values that determine the large scale structure of Brownian motion are the first components of $\mathbf{z} = (z_1,\dots,z_N)$.  

